Binary planet formation through tides

The search for satellites around exoplanets represents one of the greatest challenges in advancing the characterization of planetary systems. Currently, we can only detect massive satellites, which resemble additional planetary companions rather than rocky moons. It is not yet well understood whether such substellar pairs, known as binary planets, are common or how they form. In this study, we investigated the formation scenario for binary planets resulting from tidal dissipation during close encounters in the gravitational instability scenario. We conducted seven sets of simulations, varying the number of initial planets injected into the system from two to five, as well as the amount of energy lost due to tides. Our results demonstrate that this formation mechanism is quite efficient in producing binary planets, with an average occurrence rate for the simulated systems of 14.3%. Additionally, we present the distribution of relevant physical parameters (semi-major axis, eccentricity, mass ratios, and formation time) for planet-planet pairs. We also provide comprehensive statistics for single planets and planet-planet pairs.

==> referee_report <==
Reviewer's Comments:
Reviewer: 1

Comments to the Author
Major:

1) A few points about the numerical implementation should be better described:
 - The way tidal dissipation is implemented is not fully explicit. "...at pericentre passage we subtract the energy dissipated by tides, given by Equation 1..." I presume that this is implemented by reducing the relative velocities of the two planets, keeping the direction of the velocity vectors unchanged as well as the velocity of the barycentre of the two planets. This, or whatever the exact implementation is, should be described explicitly after Eq 1.





 
 - Eq 1 is independent of the relative velocity at infinity of the two planets, so does this apply only to near-parabolic encounters? This is probably an acceptable approximation for giant planets on wide orbits where the escape velocity from the planetary surface is much larger than the orbital velocity around the star, as the encounter velocity at infinity would then be pretty low.



 
 - There are, for every choice of parameters, 10 sets of 100 simulations. I couldn't see that there was any difference between these 10 sets, so I assume this was some way of dividing them up for e.g. running on different nodes. In which case, just say there are 1000 simulations for each parameter set.



 
 - Planet--planet collisions are a possible outcome of scattering dynamics, but aren't described in this paper and aren't listed in the table of outcomes ("collided" refers exclusively to collisions with the star). Did you check for such planet--planet collisions?





2) Several aspects of the figures should be significantly improved:
 - Figs 1 and 6: Please include error bars on the fraction of binary planets formed so the reader can evaluate the trends (I'm guessing the error would be of order 1-2%); you could also include these in the text at the relevant points. Also it's unclear what the lines are (spline fits or polynomials through all the points?). It would be better to show a regular regression line, if one is needed. Also, are different symbols really needed for the points?



 
 - Fig 2, 3, 4, 5 and 11: You have histograms labelled "cumulative distribution", which is misleading as the cumulative distribution is defined as the number of data values less than the abscissa value (i.e. the integral of the differential distribution). I'd call what you're showing the "overall distribution" or something like that, also in the associated text.



 
 - It's hard to tell by eye whether some of the distributions are the same or different (e.g., figs 4 and 5, and related text on p3). Have you considered doing say Kolmogorov--Smirnov or Anderson--Darling tests to see whether distributions are statistically consistent with each other or not?




 
 - Fig 3, 5, 8, 10: These are all histograms with logarithmic x-axes but fixed linear bin width showing the number of counts. This can be very misleading as the first bins take a disproportionate area in the plot, while a large number of datapoints at higher values can get lost as increasingly small ticks with a single value per bin. This is especially noticeable in the histograms of formation time. I think here it would be better to keep the log x-axis but show instead the cumulative distribution on the y-axis, from which the median and other quantile can be easily read off. It would also be easy then to compress these figures down to a single panel, for better comparison between the simulation sets and to save space.





Minor:

 - Title: More idiomatic would be "Binary planet formation through tides" [singular]
DONE



 - Abstract: "average occurrence rate of 14.3%": state more clearly what this means. It's the fraction of systems simulated that form a binary planet: I'd re-phrase it to avoid confusion with the occurrence rate of such objects when looking at a whole stellar population (which will be much lower).




 - p1, col2: I'm not sure the terminology for naming moons is settled, but I've previously seen Roman numerals used for the moons, not additional letters. E.g., Teachey & Kipping refer to Kepler-1625b-i.

 - p1, col2: Worth also noting that Kepler-1625 and Kepler-1708 also show dips in their light curves that may be caused by the moon candidates, as well as the TTVs mentioned (see discovery papers).

 - p1, col2, to p2: "...subsequently become a bound pair through repeated close encounters,..." surely only a single close encounter suffices? In fact, because the planets are orbiting in an external potential, energy loss in one encounter that is insufficient to result in a bound state shouldn't have a significant effect on the energy of the next encounter.

 - p2, col1, l51: "to module" -> "to modulate"

 - p3, col1, l22: "relative statistics" -> "relevant statistics"?

 - p3, col2, ll31-34: Do the binary planets tend to move inwards because they are, as a bound pair, heavier than remaining single planets and therefore tend to eject the latter?

 - Tab 2: a few entries use a comma rather than a stop as the decimal separator.

 - Fig 2, caption: "relative to the orbit of the binary" -> "that of the orbit of the binary..."

 - Fig 6: may be better with a log x axis?

 - p7 col2: "perspectives to significantly improve" -> "prospects for significantly improving"

 - p7: In the context of microlensing, you may wish to mention Hwang et al 2018 https://eur03.safelinks.protection.outlook.com/?url=https%3A%2F%2Fui.adsabs.harvard.edu%2Fabs%2F2018AJ....155..259H%2Fabstract&data=05%7C01%7Cc.lazzoni%40exeter.ac.uk%7C66e3eddb4cea4036244208dbb7cac198%7C912a5d77fb984eeeaf321334d8f04a53%7C0%7C0%7C638305853683890863%7CUnknown%7CTWFpbGZsb3d8eyJWIjoiMC4wLjAwMDAiLCJQIjoiV2luMzIiLCJBTiI6Ik1haWwiLCJXVCI6Mn0%3D%7C3000%7C%7C%7C&sdata=8Qik3Di%2BpKFLyi4njqT7ZMndIleEq4IHdn%2FAubNN590%3D&reserved=0 who found a candidate star--planet-moon microlens (although this solution was abandoned in favour of multiple sources on the basis of multi-band photometry)

 - p9, col1, l10: "apoastron" -> "apastron"

 - p9, col2: missing "\" before "lambda"


ADDITIONAL MODIFICATIONS
Beside the changes in reply to referee comments, we added a couple of sentence in Sect. 1 and Sect. 4 to mention the recent results by Fontanive et al. 2023 and Pearson et al. 2023, appeared on arxiv after the submission of the paper, which we think pertinent to the topic of our study.
